GeoGebra Discovery in Context

In our contribution we will reflect, through a collection of selected examples, on the potential impact of the GeoGebra Discovery application on different social and educational contexts.

==> eptcsdata.tex <==
\providecommand{\firstpage}{141}
\providecommand{\publicationstatus}{Jani\v{c}i\'c, Kov\'acs (Eds.): Automated Deduction in Geometry (ADG 2021)\\
EPTCS 352, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.352.16}{10.4204/EPTCS.352.16}}
\pdfoutput=1

